PhaseMO: A Universal Massive MIMO Architecture for Sustainable NextG

The rapid proliferation of devices and increasing data traffic in cellular networks necessitate advanced solutions to meet these escalating demands. Massive MIMO (Multiple Input Multiple Output) technology offers a promising approach, significantly enhancing throughput, coverage, and spatial multi-plexing. Despite its advantages, massive MIMO systems often lack flexible software controls over hardware, limiting their ability to optimize operational expenditure (OpEx) by reducing power consumption while maintaining performance. Current software-controlled methods, such as antenna muting combined with digital beamforming and hybrid beamforming, have notable limitations. Antenna muting struggles to maintain throughput and coverage, while hybrid beamforming faces hardware constraints that restrict scalability and future-proofing. This work presents PhaseMO, a versatile approach that adapts to varying network loads. PhaseMO effectively reduces power consumption in low-load scenarios without sacrificing coverage and overcomes the hardware limitations of hybrid beamforming, offering a scalable and future-proof solution. We will show that PhaseMO can achieve up to 30% improvement in energy efficiency while avoiding about 10% coverage reduction and 5dB increase in UE transmit power.

==> 1-intro.tex <==
\section{Introduction}\label{sec:introduction}
% Space resource can be a proper resource for handling data traffic
The rapid growth of bandwidth-intensive applications and the increasing user population are expected to boost cellular network traffic significantly\todo{maybe add coverage as well}. According to \cite{ericsson2024}, total mobile data traffic is forecast to grow around 20\% annually through 2029. Therefore, utilizing new free resources such as space, spatial reuse, is widely recognized as a powerful solution to address the rising demands on cellular networks. Spatial reuse can brings higher network capacity by using directional beams, allowing more beams to be concentrated in the same area to serve multiple users simultaneously while reducing interference, as illustrated in Fig. \ref{fig:intro1_fig}. Additionally, by directing the beam towards a specific direction, the beam's reach is extended, enabling it to serve users farther from the base station, thereby increasing the coverage area. 

% Explaining how spatial reuse can be achieved using large number of antennas
Employing a large number of antennas at the base station is considered a key technology for meeting increasing network traffic demands which enables using spatial reuse. This concept, initially introduced in \cite{marzetta2015massive} and \cite{marzetta2010multi}, enables higher throughput and larger coverage areas by shaping directional beams through precoding the users' data before transmission. Extensive research has focused on various precoding techniques examining throughput, hardware complexity, and cost; however, overall these techniques can generally be categorized into digital, analog, and hybrid forms. \todo{my suggestion for this paper is to define optimal behavior: in specifically you want three things to enable spatial re-use: high-throughput, low-cost, low-energy (if that fits), flexibility more specifically data proportional operational cost, }

% Explaining digital beamforming
Existing base stations employing a large number of antennas utilize digital beamforming to shape users' stream before transmission. Digital beamforming offers the highest throughput among various beamforming techniques, enabling the simultaneous forming of maximally \(N\) beams to support multiple users, as shown in Fig. \ref{fig:intro1_fig}.d)\todo{define N antennas for the entire discussion...}. However, this comes at the cost of complex hardware architecture and expensive design, primarily due to the radio frequency (RF) chain as mentioned in \cite{ahmed2016resource}. An RF chain comprises components such as analog-to-digital converters (ADC), digital-to-analog converters (DAC), data converters, mixers, etc., with ADC/DACs accounting for over 80\% of the cost of a single RF chain. \todo{summarize what digital provides and what it misses}

% explaining analog beamfomring
Analog precoding stands at the opposite side of the digital precoding in terms of hardware complexity tries to mitigate the digital beamforming hardware complexity. This technique reduces architecture complexity and cost by using a single RF chain while adding a simple RF analog network of phase shifters (PSs) with a complexity order of \(N\), where \(N\) is the number of antennas. However, this technique can only form one beam, limiting the number of served users to one and significantly reducing system throughput. Additionally, it cannot achieve a sharp beam even for that single beam, as illustrated in Fig. \ref{fig:intro1_fig}.a. \todo{summarize what analog provides and what it misses}


% HBF here 
Alternatively, hybrid beamforming technologies aim to reduce digital precoding complexity by decreasing the number of RF chains while striving to maintain performance close to that of digital beamformers. Traditional hybrid beamforming utilizes more than one RF chain and a more complex RF analog network of phase shifters (PSs) with a maximum complexity order of \(N \times R\), where \(R\) is the number of RF chains. This configuration can form up to \(R\) beams but cannot exceed this limit, as shown in Fig. \ref{fig:intro1_fig}.b) and c). Furthermore, hybrid precoding cannot achieve beams as sharp as those created by digital precoding, resulting in some throughput degradation. However, it offers better beam shaping compared to analog precoding. \todo{summarize what hybrid provides and what it misses }

%New hybrid architectures are attempting to address these drawbacks by achieving a low-complexity hybrid beamforming architecture while maintaining high performance. For instance, Gupta et al. \cite{gupta2023greenmo} employ a single RF chain with a simple RF switches network to achieve performance higher than analog beamforming. Another innovative hybrid beamforming architecture is Joint Phase-Time Arrays (JPTA), which realizes frequency-dependent analog beamforming by utilizing true-time delay elements in the analog beamforming to create frequency-dependent analog beams, in addition to the traditional phase-shifter network, thereby improving beamforming performance \cite{ratnam2022joint}.

% What we can achive using PhaseMO
In this work, we present \name, a novel low-cost hybrid beamforming architecture that combines the simplicity of analog beamforming in terms of low hardware complexity and deployment cost with the ability to achieve flexible throughput (number of beams) ranging from analog to digital precoding. Different precoding techniques vary in terms of throughput and the maximum number of beams they can create at a time, which makes each of them applicable in different network traffic loads. Networks, which fluctuate significantly over time, carry different traffic loads that can be met by employing different precoding techniques. For instance, traffic can differ from day to night when most users are inactive, so digital beamforming is suitable for meeting daytime demands, while nighttime network traffic can be satisfied with analog precoding; however, this necessitates uniform hardware architecture for all the precoding techniques. \name, which employs a single RF chain and a network of fast phase-shifters (FPSs) with a complexity order of \(N\), utilizes the analog precoding hardware architecture, enabling flexibly throughput scaling from fully analog to fully digital beamforming (Fig. \ref{fig:intro1_fig}) without having limitations of maximum number of beams rooted from hardware limitation.

% How we can achive that thing using PhaseMO
\name\ utilizes a single RF chain and a network of Fast Phase Shifters (FPSs), leveraging variable DAC/ADC sampling frequencies to create a flexible beamforming hardware architecture. To mitigate the limitation on the maximum number of beams in other beamforming architectures, \name\ requires a high sampling frequency DAC/ADC to achieve the highest throughput possible with the corresponding digital precoding design which does not increase component costs due to current trends in DAC/ADC manufacturing. \name\ uses a variable ADC/DAC sampling frequency corresponding to the number of beams, which are combined through orthogonal binary codes and then passed to the single RF chain. The combined signals are then precoded via FPSs, which affect the different precoded signals at different times, resulting in analog beamforming. For example, as shown in Fig. \ref{fig:intro2_fig}, four digitally precoded signals are first combined and passed through a \(4f_s\) DAC, then directed towards the \(N\) different antennas, each with individual FPS and analog phase control resulting in analog precoded signals. \todo{this entire paragraph needs to be re-written -- please read agrim's NSDI version to get ideas...}


% Rest of the paper
The following sections of the paper are organized as follows: Section \ref{sec:background} discusses the background and motivation of this work in detail, evaluating existing works in this field. Section \ref{sec:design} elaborates on the PhaseMO architecture, highlighting its distinct features compared to existing approaches. Section \ref{sec:evaluation} presents the evaluation of PhaseMO's performance. Finally, Section \ref{sec:discussion} explores additional features, limitations, and implications of this work.

     \begin{figure}[t]
     \centering
 \includegraphics[width=\linewidth]{figures/intro1_fig.pdf}
     \caption{(a) Analog beamforming is suitable for providing network throughput in light traffic conditions, particularly when a few users are located at the edge of the network. (b, c) Hybrid beamforming, offering higher performance, can be used to meet the medium traffic network's demand, accommodating multiple users with moderate throughput demand or a few users with high data demand. (d) Digital beamforming, which has the best performance among beamforming techniques, is an appropriate alternative to hybrid precoding to meet the throughput demand of a high traffic network.
}
     \label{fig:intro1_fig}
     \end{figure}






\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/intro2_fig.pdf}
    \caption{\name\ beamforming architecture employs a single RF chain and Fast Phase Shifters (FPSs) to replicate various beamforming techniques. It uses dynamic sampling frequency, based on the number of precoded digital signals, and combines digital streams with orthogonal binary codes passed through a DAC. The analog signals are then transmitted to \(N\) antennas, each with an FPS for phase control. This figure illustrates the process for four precoded digital signals, using a higher sampling frequency, \(4f_s\).}
    \label{fig:intro2_fig}
\end{figure}




==> 2-background.tex <==
\section{System Model}\label{sec:background}
% \begin{itemize}
%     \item MIMO background (Point-to-Point MIMO, MU-MIMO) 
%     \item massive MIMO 
%     \item existing beamforming techniques for mMIMO
%     \item Practical mMIMO architectures
% \end{itemize}

\begin{table}[t!]
\centering
\caption{Comparison of Different Beamforming Techniques}
\begin{tabular}{|l|p{1.5cm}|p{01.5cm}|p{1.8cm}|}
\hline
\textbf{Beamforming} & \textbf{Data Streams}  & \textbf{Energy\newline Efficiency} & \textbf{Adaptability\newline Future-Proof}  \\ \hline
Digital               & \cellcolor{lightgreen}Multiple                          & \cellcolor{lightred}Low          & \cellcolor{lightred}No                                          \\ \hline
Digital + AM          & \cellcolor{lightgreen}Multiple                          &\cellcolor{lightyellow} Medium          & \cellcolor{lightgreen}Yes                                         \\ \hline
Hybrid                & \cellcolor{lightyellow}Multiple\newline (Restricted)      &\cellcolor{lightyellow} Medium        & \cellcolor{lightred}No                           \\ \hline
Analog                & \cellcolor{lightred}Single                                 & \cellcolor{lightyellow} Medium           & \cellcolor{lightred}No                                           \\ \hline\hline
\textbf{\name}             & \cellcolor{lightgreen}Multiple\newline (Unrestricted)           & \cellcolor{lightgreen}High           & \cellcolor{lightgreen}Yes\newline     \\ \hline
\end{tabular}

\label{table:beamforming_comparison}
\end{table}

% this is what i want to achieve in the para
%%\subsection{Generic beamforming model for downlink}
To clarify different beamforming techniques architectures and performance, we consider a generic architecture model that can cover all existing beamforming structures, as demonstrated in Fig. \ref{fig:generic_fig}. We will show how the architectural differences in terms of hardware implementation can differentiate the mathematical model for each of them. Based on this model, which will be explained in more detail, we can write the mathematical expression for the signals emitted from the antennas based on these different parts. For now, we do not include DAC non-idealities, as we assume they will be removed by the BPF in the air interface part.

\begin{equation}
    \hat{Y}_{N\times1}(f) = \Phi_{N\times R} \Gamma_{R\times K}(f) X_{K\times 1}
\end{equation}

where \(\hat{Y}_{K\times1}\) is the emitted signal from the antennas, \(\Phi_{N\times R}\) is the analog precoding matrix, \(\Gamma_{R\times K}(f)\) is the digital precoding matrix, and \(X_{K\times 1}\) is the user's data.

Now, we can discuss the model in more detail:

\begin{itemize}
    \item \textbf{Baseband Digital Precoder}: The precoding matrix, denoted by \(\Gamma_{R\times K}(f)\), performs the baseband digital precoding over different subcarriers on users' data, denoted by the vector \(X_{K\times1}\), which has bandwidth \(B\). This precoding produces \(R\) precoded signals, each corresponding to one RF chain.

    \item \textbf{RF Chains}: The precoded digital samples (\(P_{R\times1}\)) are passed through RF chains, each of which includes a digital-to-analog converter (DAC) with sampling frequency \(f_s\) and an upconverter that transforms the baseband signal to the passband (\(f_c\)). The analog output signals are represented by \(\hat{P}_{R\times1}\) and include DAC non-idealities, such as sideband images around sampling frequency products. We will discuss this in more detail later.

    \item \textbf{RF Analog Beamformer}: This includes a network of phase shifters that perform the analog precoding on the passband signal. The analog precoding matrix (\(\Phi_{N\times R}\)), which includes unity magnitude components with different phases, maps \(R\) RF chains' analog signals to \(N\) signals, denoted by \(Y_{N \times 1}\), which are then radiated from the antennas used in the architecture.

    \item \textbf{Air Interface Part}: This section includes power amplifiers (PAs), antennas, and a bandpass filter (BPF). Positioned before the PA, the filter cleans the spectrum of non-idealities from the DAC, upconverter, and other sources. It has a bandwidth of \(B\), and is centered around \(f_c\). The filter operates on \(Y_{N\times1}\) to produce \(\hat{Y}_{N\times1}\). This configuration remains consistent across all beamforming techniques.
\end{itemize}

Finally, we can write the received signals on the user side by considering the channel effect also on the emitted signals.

\begin{equation}
    \hat{X}_{K\times1}(f) = H_{K\times N}(f) \Phi_{N\times R} \Gamma_{R\times K}(f) X_{K\times 1}
\end{equation}

where \(H_{K\times N}(f)\) is the wireless channel between \(N\) antennas and \(K\) users. In the following subsections, we will discuss how different parts differ with respect to different beamforming techniques and how these differences affect the mathematical model for each of them.



\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/generic_fig.pdf}
    \caption{A generic architecture model that can encompass all beamforming structures. This model includes four distinct parts: 
1) \textbf{Baseband Digital Precoder}, where the precoding matrix \(\Gamma_{R\times K}(f)\) performs digital precoding over subcarriers on the users' data vector \(X_{K\times 1}\) with bandwidth \(B\); 
2) \textbf{RF Chains}, where precoded digital samples \(P_{R\times 1}\) pass through RF chains, each containing a DAC with sampling frequency \(f_s\) and an upconverter to the passband \(f_c\), resulting in analog output signals \(\hat{P}_{R\times 1}\) including DAC non-idealities; 
3) \textbf{RF Analog Beamformer}, consisting of phase shifters that perform analog precoding on the passband signal, mapping \(R\) RF chains' analog signals to \(N\) signals \(Y_{N\times 1}\) radiated from the antennas; 
4) \textbf{Air Interface Part}, featuring power amplifiers, antennas, and a bandpass filter that cleans the spectrum of non-idealities, operating on \(Y_{N\times 1}\) to produce \(\hat{Y}_{N\times 1}\) with a bandwidth of \(B\) centered around \(f_c\).}
    \label{fig:generic_fig}
\end{figure*}

\subsubsection{Digital beamforming} 
In a digital beamforming architecture, all the precoding is performed on digital symbols, and there is no analog precoder. Consequently, there must be an equal number of RF chains and antennas. This implies \(R = N\), \(\Phi_{N\times R} = \Phi_{N \times N}\), and \(\Gamma_{R\times K} = \Gamma_{N\times K}\). Thus, we can rewrite the mathematical expression for the signals emitted from the antennas for digital beamforming using Eq. 1.

\begin{equation}
    \hat{Y}_{N\times1} = \Gamma_{N\times K}(f) X_{K\times 1}
\end{equation}

\subsubsection{Analog beamforming} 
Analog beamformers, which are structurally different from digital beamformers, do not utilize any digital precoder. Instead, a single RF chain is employed to convert digital symbols into an analog signal, limiting the architecture to support only one user's data transmission at a time (\(R = K = 1\), \(X_{K \times 1} = X_{1 \times 1}\), and \(\Gamma_{1 \times 1} = 1\)). This constraint significantly reduces the system's throughput. In the analog domain, a network of phase shifters is used for precoding. This network comprises as many phase shifters as there are antennas (\(N\)) in the architecture, resulting in the analog precoder matrix being an \(N \times 1\) vector. Therefore, the mathematical expression for the analog beamformer can be rewritten with respect to Eq. 1 as follows:

\begin{equation}
    \hat{Y}_{N \times 1} = \Phi_{N \times 1} X_{1 \times 1}
\end{equation}



\subsubsection{Hybrid beamforming} 
Hybrid beamforming, as the name suggests, includes both a digital precoder and an analog beamformer. Therefore, the generic structure depicted in Fig. \ref{fig:generic_fig} accurately represents a hybrid beamformer architecture. This architecture includes \(R\) RF chains, which convert the digitally precoded symbols using \(\Gamma_{R\times K}(f)\) into analog signals. These analog signals are then beamformed via a network of phase shifters and radiated from \(N\) antennas. The analog network can be categorized into two types: a) Fully connected, and b) Partially connected. In a fully connected architecture, all \(R\) RF chains are connected to all \(N\) antennas. However, in the partially connected architecture, each RF chain is connected to a subset of antennas. The mathematical representation of the radiated signals from the antennas for a hybrid beamformer follows the same generic mathematical model. However, in a partially connected hybrid beamformer, only a few elements of the analog beamforming matrix \(\Phi_{N\times R}\) are non-zero, indicating the connections between RF chains and antennas.


\begin{equation}
    \hat{Y}_{N\times1} = \Phi_{N\times R} \Gamma_{R\times K}(f) X_{K\times 1}
\end{equation}

In conclusion, different hardware structure for RF chains part and the analog precoder results in different beamforming architectures, in the next section, we will show how PhaseMO can be represented as a viable alternative for all the beamforming techniques by keeping the hardware complexity of an analog beamforming structure.




% \begin{table}[h!]
% \centering
% \caption{Comparison of Different Beamforming Techniques}
% \begin{tabular}{|l|l|p{0.75cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% \textbf{Beamforming} & \textbf{Complexity} & \textbf{Cost} & \textbf{Inter-user\newline Interference} & \textbf{Data Streams} \\ \hline
% Digital              & High                & High          & Low                               & Multiple              \\ \hline
% Digital + AM         & Medium               & High          & Low                               & Multiple              \\ \hline
% Analog               & Low                 & Low           & High                              & Single                \\ \hline
% Hybrid               & Medium              & Medium        & Medium                            & Multiple\newline (Restricted) \\ \hline
% PhaseMO              & Low                 & Low           & Flexible\newline    & Flexible\newline (Unrestricted) \\ \hline
% \end{tabular}

% \label{table:beamforming_comparison}
% \end{table}


% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|}
%         \hline
%         Column 1 & Column 2 & Column 3 \\
%         \hline
%         \cellcolor{lightred} R1C1 & R1C2 & \cellcolor{lightgreen} R1C3 \\
%         \hline
%         R2C1 & \cellcolor{lightyellow} R2C2 & R2C3 \\
%         \hline
%         \cellcolor{lightgreen} R3C1 & R3C2 & \cellcolor{lightred} R3C3 \\
%         \hline
%     \end{tabular}
%     \caption{A table with colored cells}
%     \label{tab:colored_cells}
% \end{table}

==> 3-design.tex <==
\section{Design}\label{sec:design}
In this section, we first provide an overview of existing beamforming architectures for downlink. Then, the \name\ design will be presented in detail for downlink, along with a discussion of \name's innovations and requirements. We begin by examining a generic beamforming architecture and a generic mathematical model applicable to all beamforming techniques (digital beamforming, analog beamforming, and hybrid beamforming). Following this, we will discuss the differences among these techniques in terms of complexity in various parts of the architecture (baseband digital precoder, RF chains, and analog RF beamformer) and their mathematical models. Then, we will demonstrate the mathematical foundation of \name\ and illustrate how \name\ relates to other beamforming techniques.

 \todo{Discuss the \name architecture and how it contrasts with existing MIMO architecture first without maths.}
\subsection{Generic beamforming model for downlink}
To better clarify the different beamforming techniques architectures and performance, we consider a generic architecture model that can cover all beamforming structures, as demonstrated in Fig. \ref{fig:generic_fig}. We will show how the architectural differences in terms of hardware implementation can differentiate the mathematical model for each of them. Based on this model, which will be explained in more detail, we can write the mathematical expression for the signals emitted from the antennas based on these different parts. For now, we do not include DAC non-idealities, as we assume they will be removed by the BPF in the air interface part.

\begin{equation}
    \hat{Y}_{N\times1}(f) = \Phi_{N\times R} \Gamma_{R\times K}(f) X_{K\times 1}
\end{equation}

where \(\hat{Y}_{K\times1}\) is the emitted signal from the antennas, \(\Phi_{N\times R}\) is the analog precoding matrix, \(\Gamma_{R\times K}(f)\) is the digital precoding matrix, and \(X_{K\times 1}\) is the user's data.

Now, we can discuss the model in more detail:

\begin{itemize}
    \item \textbf{Baseband Digital Precoder}: The precoding matrix, denoted by \(\Gamma_{R\times K}(f)\), performs the baseband digital precoding over different subcarriers on users' data, denoted by the vector \(X_{K\times1}\), which has bandwidth \(B\). This precoding produces \(R\) precoded signals, each corresponding to one RF chain.

    \item \textbf{RF Chains}: The precoded digital samples (\(P_{R\times1}\)) are passed through RF chains, each of which includes a digital-to-analog converter (DAC) with sampling frequency \(f_s\) and an upconverter that transforms the baseband signal to the passband (\(f_c\)). The analog output signals are represented by \(\hat{P}_{R\times1}\) and include DAC non-idealities, such as sideband images around sampling frequency products. We will discuss this in more detail later.

    \item \textbf{RF Analog Beamformer}: This includes a network of phase shifters that perform the analog precoding on the passband signal. The analog precoding matrix (\(\Phi_{N\times R}\)), which includes unity magnitude components with different phases, maps \(R\) RF chains' analog signals to \(N\) signals, denoted by \(Y_{N \times 1}\), which are then radiated from the antennas used in the architecture.

    \item \textbf{Air Interface Part}: This section includes power amplifiers (PAs), antennas, and a bandpass filter (BPF). Positioned before the PA, the filter cleans the spectrum of non-idealities from the DAC, upconverter, and other sources. It has a bandwidth of \(B\), and is centered around \(f_c\). The filter operates on \(Y_{N\times1}\) to produce \(\hat{Y}_{N\times1}\). This configuration remains consistent across all beamforming techniques.
\end{itemize}

Finally, we can write the received signals on the user side by considering the channel effect also on the emitted signals.

\begin{equation}
    \hat{X}_{K\times1}(f) = H_{K\times N}(f) \Phi_{N\times R} \Gamma_{R\times K}(f) X_{K\times 1}
\end{equation}

where \(H_{K\times N}(f)\) is the wireless channel between \(N\) antennas and \(K\) users. In the following subsections, we will discuss how different parts differ with respect to different beamforming techniques and how these differences affect the mathematical model for each of them.



\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/generic_fig.pdf}
    \caption{A generic architecture model that can encompass all beamforming structures. This model includes four distinct parts: 
1) \textbf{Baseband Digital Precoder}, where the precoding matrix \(\Gamma_{R\times K}(f)\) performs digital precoding over subcarriers on the users' data vector \(X_{K\times 1}\) with bandwidth \(B\); 
2) \textbf{RF Chains}, where precoded digital samples \(P_{R\times 1}\) pass through RF chains, each containing a DAC with sampling frequency \(f_s\) and an upconverter to the passband \(f_c\), resulting in analog output signals \(\hat{P}_{R\times 1}\) including DAC non-idealities; 
3) \textbf{RF Analog Beamformer}, consisting of phase shifters that perform analog precoding on the passband signal, mapping \(R\) RF chains' analog signals to \(N\) signals \(Y_{N\times 1}\) radiated from the antennas; 
4) \textbf{Air Interface Part}, featuring power amplifiers, antennas, and a bandpass filter that cleans the spectrum of non-idealities, operating on \(Y_{N\times 1}\) to produce \(\hat{Y}_{N\times 1}\) with a bandwidth of \(B\) centered around \(f_c\).}
    \label{fig:generic_fig}
\end{figure*}

\subsubsection{Digital beamforming} 
In a digital beamforming architecture, all the precoding is performed on digital symbols, and there is no analog precoder. Consequently, there must be an equal number of RF chains and antennas. This implies \(R = N\), \(\Phi_{N\times R} = \Phi_{N \times N}\), and \(\Gamma_{R\times K} = \Gamma_{N\times K}\). Thus, we can rewrite the mathematical expression for the signals emitted from the antennas for digital beamforming using Eq. 1.

\begin{equation}
    \hat{Y}_{N\times1} = \Gamma_{N\times K}(f) X_{K\times 1}
\end{equation}

\subsubsection{Analog beamforming} 
Analog beamformers, which are structurally different from digital beamformers, do not utilize any digital precoder. Instead, a single RF chain is employed to convert digital symbols into an analog signal, limiting the architecture to support only one user's data transmission at a time (\(R = K = 1\), \(X_{K \times 1} = X_{1 \times 1}\), and \(\Gamma_{1 \times 1} = 1\)). This constraint significantly reduces the system's throughput. In the analog domain, a network of phase shifters is used for precoding. This network comprises as many phase shifters as there are antennas (\(N\)) in the architecture, resulting in the analog precoder matrix being an \(N \times 1\) vector. Therefore, the mathematical expression for the analog beamformer can be rewritten with respect to Eq. 1 as follows:

\begin{equation}
    \hat{Y}_{N \times 1} = \Phi_{N \times 1} X_{1 \times 1}
\end{equation}



\subsubsection{Hybrid beamforming} 
Hybrid beamforming, as the name suggests, includes both a digital precoder and an analog beamformer. Therefore, the generic structure depicted in Fig. \ref{fig:generic_fig} accurately represents a hybrid beamformer architecture. This architecture includes \(R\) RF chains, which convert the digitally precoded symbols using \(\Gamma_{R\times K}(f)\) into analog signals. These analog signals are then beamformed via a network of phase shifters and radiated from \(N\) antennas. The analog network can be categorized into two types: a) Fully connected, and b) Partially connected. In a fully connected architecture, all \(R\) RF chains are connected to all \(N\) antennas. However, in the partially connected architecture, each RF chain is connected to a subset of antennas. The mathematical representation of the radiated signals from the antennas for a hybrid beamformer follows the same generic mathematical model. However, in a partially connected hybrid beamformer, only a few elements of the analog beamforming matrix \(\Phi_{N\times R}\) are non-zero, indicating the connections between RF chains and antennas.


\begin{equation}
    \hat{Y}_{N\times1} = \Phi_{N\times R} \Gamma_{R\times K}(f) X_{K\times 1}
\end{equation}

In conclusion, different hardware structure for RF chains part and the analog precoder results in different beamforming architectures, in the next section, we will show how PhaseMO can be represented as a viable alternative for all the beamforming techniques by keeping the hardware complexity of an analog beamforming structure.

\subsection{\name\ in downlink} 
%\todo{Probably easier to discuss \name uplink first and then downlink?}
In this section, we present \name's architecture for downlink communication and explore its differences across the three components of a generic beamforming architecture (the air interface part remains the same). We will demonstrate that \name's final mathematical model aligns with all other beamformings, but with significantly reduced design complexity. Specifically, \name utilizes only a single RF chain and features an RF analog beamformer with significantly low-complexity. 

Here, we will explain how \name\ differs architecturally from traditional beamforming methods. In Fig. \ref{fig:PhaseMO_fig}, a simple use case of both traditional beamforming and \name\ is illustrated. \name\ employs a digital interleaver to combine all precoded signals into one, which is then passed through a DAC operating at a higher frequency proportional to the number of digitally precoded signals. In contrast, traditional structures require as many RF chains as there are precoded signals. Additionally, \name\ uses a fast phase shifter at the output of each antenna to beamform the analog signal, whereas traditional architectures use time-invariant phase shifters because the exact precoded symbols are passed through the DACs.

     \begin{figure}[t]
     \centering
 \includegraphics[width=\linewidth]{figures/PhaseMO_explanation_fig.pdf}
     \caption{
Traditional and \name\ beamforming architectures: a) Traditional beamforming architecture utilizes multiple RF chains, each corresponding to a precoded signal, followed by time-invariant phase shifters at each antenna. b) \name\ architecture combines all precoded signals into one via a digital interleaver, then passes it through a DAC operating at a higher frequency. Fast phase shifters at each antenna beamform the combined analog signal.}
     \label{fig:phaseMO_explanation}
     \end{figure}

In the subsequent subsections, we will first examine \name's digital component, which introduces a novel element not present in earlier beamforming architectures, known as the \textit{Sample Interleaver}. Next, we will detail the analog components of the architecture, which includes fast phase-shifters (FPSs), and the air interface part, which remains consistent with previous designs. For each component, we will also provide a mathematical explanation of how different operations influence the signal, ultimately revealing their impact together on the emitted signals from the antennas.



\subsubsection{Digital part}
The digital segment of \name\ includes a digital precoder, represented by the matrix \(\Gamma_{V\times K}(f)\), which generates \(V\) different digitally precoded signals that \(V\) shows the number of virtual RF chains, we want to model using only single physical RF chain. These \(V\) digital symbols are then interleaved using a sample interleaver block. The interleaved signal is subsequently passed through a DAC with a sampling frequency of \(f'_s=Vf_s\) which \(f_s\) is DAC sampling rate we considered for other beamforming techniques shown in Fig. \ref{fig:generic_fig}. The mathematical representation of the digital part can be described in the following steps.

As in previous precoding steps, we utilize a digital precoder that transforms the raw user data into digitally precoded data, maintaining the same length as the original user data. This can be expressed mathematically as:
\begin{equation}
    \mathbf{P}_{V\times 1} = \Gamma_{V\times K}(f) \mathbf{X}_{K \times 1}
\end{equation}
where \(\mathbf{X}_{K \times 1}\) is the vector of raw user data and \(\Gamma_{V\times K}(f)\) is the digital precoding matrix.

Next, we employ a sample interleaver to interleave the digitally precoded time-domain symbols. This interleaving process can be represented as:
\begin{equation}
    z[n] = [p_1[1], p_2[1], \ldots, p_V[1], p_1[2], p_2[2], \ldots, p_V[2], \ldots]
\end{equation}
where \(p_v[m]\) denotes the \(m\)-th sample of the \(v\)-th digitally precoded time-domain symbol.

To transform the interleaved signal into the frequency domain, we can write:
\begin{equation}
    Z(f) = P_{1}(f) + e^{-\frac{j 2 \pi T_s}{V}} P_{2}(f) + \cdots + e^{-\frac{j 2 \pi (V-1) T_s}{V}} P_{V}(f)
\end{equation}
where \(e^{-\frac{j v 2 \pi T_s}{V}}\) represents the frequency-domain phase shift due to the time-domain delay for \(v\)-th precoded symbol vector.

Finally, we account for the non-idealities of the DAC by modeling its effect as a function \(A(f)\) that introduces sidebands at the sampling frequency \(f'_s=Vf_s\) with a \( \text{sinc}(ff'_s) \) roll-off factor. The analog signal in the frequency domain, incorporating these non-idealities, can be expressed as:
\begin{equation}
    \hat{Z}(f) = A(Z(f))
\end{equation}
where \(A(f)\) encapsulates the DAC's non-ideality effects.


\subsubsection{Analog precoder}
The analog precoder employs one Fast Phase Shifter (FPS) per antenna. Each FPS generates a periodic signal with a period of \(VT'_s\), where \(V\) is the number of users supported by the base station and \(T'_s = \frac{1}{f'_s}\), with \(f'_s\) being the DAC sampling frequency. We can express the mathematical representation of the analog precoder in the following steps.

First, we define the signal generated by a single FPS over one period. This can be modeled as a summation of shifted pulses with constant phases:

\begin{equation}
    f_n(t) = \sum_{v=0}^{V-1} e^{j\Phi_{nv}} \Pi_{T'_s}(t - vT'_s - \frac{T'_s}{2})
\end{equation}

where \(f_n(t)\) is the time-variant signal produced by the FPS at the \(n\)-th antenna, and \(\Phi_{nv}\) is the \(v\)-th phase produced by the \(n\)-th antenna FPS.

Next, we extend \(f_n(t)\) to account for its periodic nature:

\begin{equation}
    f_n(t) = \sum_{i=-\infty}^{\infty} \sum_{v=0}^{V-1} e^{j\Phi_{nv}} \Pi_{T'_s}(t - iVT'_s - vT'_s - \frac{T'_s}{2})
\end{equation}

Here, \(VT'_s\) represents the duration of one period.

To convert the time-domain signal to the frequency domain, we rewrite the time-domain signal to include the convolution of the pulse with an impulse train:

\begin{equation}
    f_n(t) = \sum_{v=0}^{V-1} e^{j\Phi_{nv}} \sum_{i=-\infty}^{\infty} \left(\Pi_{T'_s}(t - vT'_s - \frac{T'_s}{2}) * \delta(t - iVT'_s)\right)
\end{equation}

The frequency-domain representation of \(f_m(t)\) can then be derived as:


    \begin{multline}
    F_n(f) = \sum_{v=0}^{V-1} e^{j\Phi_{nv}} \sum_{i=-\infty}^{\infty} \mathscr{F}\left[\delta(t - iVT'_s)\right] \mathscr{F}\left[\Pi_{T_s}(t - vT'_s - \frac{T'_s}{2})\right] \\
    = \sum_{v=0}^{V-1} e^{j\Phi_{nv}} \sum_{i=-\infty}^{\infty} \frac{1}{VT'_s} \delta\left(f - \frac{i}{VT'_s}\right) T'_s e^{-j 2\pi f (vT'_s + \frac{T'_s}{2})} \text{sinc}(fT'_s) \\
    = \sum_{v=0}^{V-1} \frac{1}{V} e^{j\Phi_{nv}} \sum_{i=-\infty}^{\infty} \delta\left(f - \frac{i}{VT'_s}\right) e^{-j \frac{2\pi i}{VT'_s} (vT'_s + \frac{T'_s}{2})} \text{sinc}\left(\frac{i}{V}\right)
    \end{multline}


In the following section, we will present the end-to-end mathematical derivation of \name's architecture, incorporating the previously discussed components.


\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/PhaseMO_fig.pdf}
    \caption{Architecture of the PhaseMO system, including key components as follows:
1) \textbf{Baseband Digital Precoder}, where the $V \times K$ precoding matrix $\Gamma_{V \times K}(f)$ performs digital precoding over subcarriers on the users' data vector $X_{K \times 1}$ with bandwidth $B$;
2) \textbf{Interleaver}, which organizes the $V$ digitally precoded symbols into a sequence for processing;
3) \textbf{RF Chain}, where the interleaved digital samples $Z$ pass through a single RF chain with a DAC having a sampling frequency $f_s$ and an upconverter to the passband $f_c$, resulting in analog output signals $\hat{Z}$ with potential DAC non-idealities;
4) \textbf{RF Analog Beamformer}, comprising one fast phase shifter (FPS) per antenna that generates a time-variant signal $f_n(t)$, forming the analog precoding matrix $\Phi_{N \times K}$, which maps the RF chain’s analog signals to $N$ output signals $Y_{N \times 1}$ radiated by the antennas;
5) \textbf{Air Interface Part}, including power amplifiers (PAs), antennas, and a bandpass filter with bandwidth $B$ centered around $f_c$, cleaning the spectrum of non-idealities, processing $Y_{N \times 1}$ to produce $\hat{Y}_{N \times 1}$.}
    \label{fig:PhaseMO_fig}
\end{figure*}


\subsubsection{Unified \name\ design}
In this section, we unify the previously discussed analog and digital components of the architecture and incorporate the effects of the air interface. Specifically, we address how the air interface, including the bandpass filter, impacts the signal. The bandpass filter is crucial for eliminating non-idealities such as DAC image artifacts from the signal spectrum and should have a bandwidth of \(2B\), where \(B\) represents the baseband signal bandwidth.

First, we express the time-domain signal at the output of the Fast Phase Shifter (FPS) and then derive its corresponding frequency-domain representation:

\begin{equation}
    y_n(t) = \hat{z}(t) \times f_n(t) \xrightarrow{\mathscr{F}} Y_n(f) = \hat{Z}(f) * F_n(f)
\end{equation}

Here, \(\hat{Z}(f)\) and \(F_n(f)\) are derived in Eqs. (8) and (14), respectively. Substituting these into the expression gives:

\begin{multline}
    Y_n(f) = \sum_{v=0}^{V-1} \frac{1}{V} e^{j\Phi_{nv}} \\
    \times \sum_{i=-\infty}^{\infty} A(Z(f))\bigg|_{f=f-\frac{i}{VT'_s}} \\
    \times e^{-j \frac{2\pi i}{VT'_s}} \text{sinc}\left(\frac{i}{V}\right)
\end{multline}

This expression indicates that the final spectrum, which is passed through each bandpass filter, includes the DAC output spectrum and a \(\frac{if'_s}{V}\) shifted versions of that spectrum, resulting from the switching effect. The bandpass filter will remove other sidebands, but we need to determine the exact output of the filter.

DAC image artifacts are located at \(f'_s\) frequencies. For values of \(i\) that are multiples of \(V\) (\(i = \ldots, -2V, -V, 0, V, 2V, \ldots\)), these images will be shifted into the band that the bandpass filter will pass. Consequently, the output of the bandpass filter can be determined as:

\begin{multline}
    \hat{Y}_n(f) = \sum_{v=0}^{V-1} \frac{1}{V} e^{j\Phi_{nv}} \sum_{i=-\infty, i=nV}^{\infty} A(Z(f))\bigg|_{f=f-\frac{i}{VT'_s}} \\
    e^{-j \frac{2\pi i}{VT'_s}(vT'_s+\frac{T'_s}{2})} \text{sinc}\left(\frac{i}{V}\right)
\end{multline}

For all \(i \neq 0\), the expression evaluates to zero, and for \(i=0\), we have \(A(Z(f)) \approx Z(f)\). Therefore:

\begin{equation}
    \hat{Y}_n(f) = \sum_{v=0}^{V-1} \frac{1}{V} e^{j\Phi_{nv}} Z(f)
\end{equation}

Combining Eqs. (5), (7), and (18), we derive the signal radiated from the antennas:

\begin{multline}
    \hat{Y}_n(f) = \sum_{v=0}^{V-1} \frac{1}{V} e^{j\Phi_{nv}} \left(Y_{1}(f) + e^{-\frac{j 2 \pi T_s}{V}} Y_{2}(f) \right. \\
    \left. + \cdots + e^{-\frac{j 2 \pi (V-1) T_s}{V}} Y_{V}(f)\right)
\end{multline}

By substituting \(Y_i(f)\) with \(Y_i(f) e^{-\frac{j 2 \pi (i-1) T_s}{K}}\) which can be done digitally after the precoding and before interleaving, we can express the summation in matrix form:

\begin{equation}
    \hat{Y}_{N\times 1}(f) = \frac{1}{V} \Phi_{N\times V} Y_{V \times 1}(f)
\end{equation}

Furthermore, using Eq. (5) to clarify the final radiated signal on the user side, we get:
\begin{equation}
    \hat{Y}_{N\times 1} = \frac{1}{V} \Phi_{N\times V} \Gamma_{V\times K}(f) \mathbf{X}_{K \times 1}
\end{equation}

Finally, if we consider channel, we can figure out what signal will be received on the user side that can be written as follows: 

\begin{equation}
    \hat{X}_{K\times 1} = \frac{1}{V} H_{K \times N}(f) \Phi_{N\times V} \Gamma_{V\times K}(f) \mathbf{X}_{K \times 1}
\end{equation}

We now aim to further explain the equation derived for the signal emitted from the antennas and discuss how PhaseMO can relate to the other beamforming techniques mentioned earlier. For this, we refer to Eq. 19.

\begin{itemize}
    \item \textbf{V=M}: In this case, the final equation can be written as follows:
    \begin{equation}
        \hat{Y}_{N\times 1} = \Phi_{N\times V} \Gamma_{V\times K}(f) \mathbf{X}_{K \times 1}
    \end{equation}
    This equation is exactly similar to what we already derived for a digital beamformer, which uses the same number of RF chains and antennas (Eq. 2). In this scenario, the fast phase shifter for each antenna only needs to create zero phase shift.
    
    \item \textbf{V=1}: In this case, the final equation can be written as follows:
    \begin{equation}
        \hat{Y}_{N\times 1} = \Phi_{N\times 1} \mathbf{X}_{1 \times 1}
    \end{equation}
    We can observe that this equation is in the same form as that for an analog beamformer, which uses just one RF chain (Eq. 3). This shows that PhaseMO with \(V=1\) can model an analog beamformer. Here, the fast phase shifter for each antenna only needs to add a constant, time-invariant phase to the single RF chain signal.
    
    \item \textbf{V=R}: In this case, where we consider \(V\) as a number that can model the hybrid beamforming architecture, the final equation can be written as follows:
    \begin{equation}
        \hat{Y}_{N\times 1} = \Phi_{N\times R} \Gamma_{R\times K}(f) \mathbf{X}_{K \times 1}
    \end{equation}
    This equation aligns with the form we have for a hybrid beamformer. It shows that PhaseMO with \(V=R\) can model a hybrid beamformer. Here, the fast phase shifter for each antenna must produce an \(R\)-periodic phase shift on its input signal.
\end{itemize}

In conclusion, PhaseMO with just a single RF chain can be a viable alternative to all the beamforming structures discussed. 



     \begin{figure}[h]
     \centering
 \includegraphics[width=\linewidth]{figures/design_BPF.png}
     \caption{Commercial Transition Plan for Each  Component.}
     \label{fig:spectrum}
 \end{figure}



\begin{comment}
    
If we denote the analogue received signal for the user number \(k\) as \( y_k(t) \), then the digital signal at the output of the ADC can be named as \( y_k[n] \). The received signal at the receiver side can be expressed as:

\[y_k(t)=\Sigma_{m=1}^{M} w_m(t)*h_{km}(t)\]

where \( M \) is the total number of antennas at the base station, \( w_m(t) \) is the signal radiated from the \( m \)-th antenna, and \( h_{km}(t) \) represents the channel between the \( k \)-th user and the \( m \)-th antenna.

On the transmitter side, we perform analogue phase-shifting \( s_{mk}(t) \) on the analogue signals that are digitally precoded in the baseband \( z(t) \):


\[w_m(t)=\Sigma_{k=1}^{K}s_{mk}(t)z(t)\]

Thus, the received signal can be written as:

\[y_k(t)=\Sigma_{m=1}^M\Sigma_{k=1}^{K}(s_{mk}(t)z(t))*h_{km}(t)\]

For the sampled digital signal, we have:

\[y_k[n]=y_k(\frac{nT_s}{K})=\]
\[\Sigma_{m=1}^M\Sigma_{k=1}^{K}(s_{mk}(\frac{nT_s}{K})z(\frac{nT_s}{K}))*h_{km}(\frac{nT_s}{K})\]

Further, we can express the signal as:

\[y_k[i]=y_k(iT_s+\frac{kT_s}{K})=\]
\[\Sigma_{m=1}^M\Sigma_{k=1}^{K}(s_{mk}(iT_s+\frac{kT_s}{K})z(iT_s+\frac{kT_s}{K}))*h_{km}(iT_s+\frac{kT_s}{K})\]

Considering the phase-shifting and channel consistency over a symbol period:

\[s_{mk}((i-1)T_s+\frac{kT_s}{K})=s_{mk}(iT_s+\frac{kT_s}{K})=s_{mk}((i+1)T_s+\frac{kT_s}{K})=s_{mk}\]

\[h_{mk}(iT_s)=h_{mk}(iT_s+\frac{kT_s}{K})=...=h_{mk}(iT_s+\frac{(K-1)T_s}{K})=h_{mk}(i)\]

Thus, the received signal can be simplified to:

\[y_k[i]=\Sigma_{m=1}^M\Sigma_{k=1}^{K}z_k(iT_s+\frac{kT_s}{K})*(h_{km}[i]s_{mk})\]

In the frequency domain, we have:

\[Y_k[f]=\Sigma_{m=1}^M\Sigma_{k=1}^{K}Z_k[f]e^{-\frac{j2\pi kT_s }{K}f}(H_{km}[f]S_{mk})\]

We can rewrite the final result in a matrix form:

\[Y_{K\times 1}[f]=H_{K\times M}[f]S_{M\times K}\^{Z}_{K\times 1}[f]\]
\[\^{Z}_{K\times 1}[f]=Z_k[f]e^{-\frac{j2\pi kT_s }{K}f}\]

Then, if we precode the signal in the following way, we can easily receive the user's streams on the receiver side:

\[\^{Z}_{K\times 1}[f]=(H_{K\times M}[f]S_{M\times K})^{-1}X_{K\times 1}[f] \xrightarrow{} Y_{K\times 1}[f]=X_{K\times 1}[f]\]



\end{comment}
    
